Multi-modal Program Inference: a Marriage of Pre-trainedLanguage Models and Component-based Synthesis

Multi-modal program synthesis refers to the task of synthesizing programs (code) from their specification given in different forms, such as a combination of natural language and examples. Examples provide a precise but incomplete specification, and natural language provides an ambiguous but more "complete" task description. Machine-learned pre-trained models (PTMs) are adept at handling ambiguous natural language, but struggle with generating syntactically and semantically precise code. Program synthesis techniques can generate correct code, often even from incomplete but precise specifications, such as examples, but they are unable to work with the ambiguity of natural languages. We present an approach that combines PTMs with component-based synthesis (CBS): PTMs are used to generate candidates programs from the natural language description of the task, which are then used to guide the CBS procedure to find the program that matches the precise examples-based specification. We use our combination approach to instantiate multi-modal synthesis systems for two programming domains: the domain of regular expressions and the domain of CSS selectors. Our evaluation demonstrates the effectiveness of our domain-agnostic approach in comparison to a state-of-the-art specialized system, and the generality of our approach in providing multi-modal program synthesis from natural language and examples in different programming domains.

==> Figs/rank.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\algsetup{
    linenosize=\Small,
    linenodelimiter = {:}
}
\begin{figure}
%
%
%
%
\begin{minipage}{0.48\textwidth}
%
%
%
\begin{subfigure}[b]{\textwidth}
\begin{mdframed}[backgroundcolor=grey12,linecolor=grey4,innerleftmargin=0.2cm]
\footnotesize
 \begin{algorithmic}[1]
  {\customline{}
  \STATE $\func{rank}$ $(T,\model):=$ 
  \STATE  \ \ \ \ $f_1 = \lambda t.\; \func{eucDist}(\model,t)$ 
  \STATE  \ \ \ \ $f_2 = \lambda t.\; (\sum_{m\in\model}\mathtt{lev}(t,m))/|\model|)$ 
  \STATE  \ \ \ \ \textbf{return} $T.\mathtt{orderBy}(f_1,f_2)$
%  \STATE  \ \ \ \ $v_2 := v_1.\mathtt{order}(\lambda p. \sqrt{\sum_{o\in\op}(\mathtt{cnt}(p,o)-\func{cnt}(\model,o))^2})$ 
  }
 \end{algorithmic}
 \end{mdframed}
  \vspace{-1.2mm}
 \caption{ranking candidates}
  \vspace{4mm}
  \label{subfig:rank}
 \end{subfigure}
%
%
%
%
\\
%
\begin{subfigure}[b]{\textwidth}
\begin{mdframed}[backgroundcolor=grey12,linecolor=grey4,innerleftmargin=0.2cm]
\footnotesize
 \begin{algorithmic}[1]
  {\customline{}
  \STATE $\func{eucDist}$ $(\model,t):=$ 
  \STATE  \ \ \ \ $<\!\!v_1,\dots,v_n\!\!> := \mathtt{opVec}(t)$
  \STATE  \ \ \ \ $<\!\!v'_1,\dots,v'_n\!\!> := (\sum_{m\in\model} \mathtt{opVec}(m))/|\model|$
  \STATE  \ \ \ \ \textbf{return} $\sqrt{\sum_{1\leq i\leq n}(v_i-v'_i)^2}$
  }
 \end{algorithmic}
 \end{mdframed}
  \vspace{-1.2mm}
 \caption{standard Euclidean distance}
  \vspace{4mm}
  \label{subfig:eucDist}
 \end{subfigure}
%
%
%
%
\\
%
%
%
%
%
\begin{subfigure}[b]{\textwidth}
\scriptsize
%\footnotesize
\begin{mdframed}[backgroundcolor=grey12,linecolor=grey4,innerleftmargin=0.2cm]
{\renewcommand{\arraystretch}{1}%
\begin{tabular}{p{1.5cm}p{4.2cm}}
  \vspace{  0.06mm}$\mathtt{opVec}(t):$ &\scriptsize  { returns a vector composed of the number of each operator in $t$} \\     \arrayrulecolor{grey8}\hline
   \vspace{  0.06mm}$\mathtt{orderBy}(f_1,f_2)$:&\scriptsize   { returns a lexicographically ordered list based on given score functions $f_1$ and $f_2$}\\     \arrayrulecolor{grey8}\hline
  \vspace{  0.06mm} $\mathtt{lev}(t_1,t_2)$:& \scriptsize   {returns the Levenshtein distance between string representations of $t_1$ and $t_2$ } 
\end{tabular}
}
\end{mdframed}
\caption{constants and auxiliary functions}
\label{subfig:aux}
 \end{subfigure}
%
%
%
%
%
%
%
\end{minipage}
%
%
%
%
%\
  \caption{Component-based synthesis algorithm parameterized on a DSL $\lang$ %$\lang:=(\sort,\const,\op,\mathtt{S}^\circ,\sigin,\sigret)$
  }
  \label{alg:over}
  \label{fig:alg}
%
%
%
%

\end{figure}


==> Reviews/Final-response.tex <==
We thank the reviewing committee for their detailed reviews and helpful comments. We will incorporate all suggestions for improvement of the paper. 

------------
#1 OVERVIEW
------------
Here we give a short summary of the main points that we want to convey to all the reviewers:

------------------------------------
## Claims of being language-agnostic 
------------------------------------
We agree that we may have stressed the generality of our approach perhaps too strongly and we will clarify its scope and expected limitations. Our goal is not to claim that our approach can be directly applied to any arbitrary language, but only that it is not specialized to one particular language, and we support this by showing its applicability and benefits in two very different programming domains. We discuss some expected limitations in points C and D in section 7. In particular, our approach does rely on a well-defined notion of input-output examples that the user can easily provide, and evaluation of sub-expressions on the inputs should produce well-defined outputs that can be compared during synthesis (using the notions of semantic equivalence).

We do not assume that the inputs of a program and the parse tree of the program follow the same hierarchical decomposition (e.g. in CSS there is no such direct correspondence), but it is true that our approach is more effective when sub-expressions produce meaningful semantic values in a compositional manner. We have discussed expected improvements to handle other domains such as Pandas, and in practice we do not expect to immediately scale to large programs in highly expressive general purpose programming languages such as Python or Java. However, it is an interesting research direction to build upon our ideas here: for instance, we have done initial experiments on small code snippets in C# with promising results, which suggest a compositional approach to multi-modal synthesis may be valuable: instead of just input-output examples, if the user can provide “traces” of examples over some pseudo-code in natural language (similar to “trace tables” students learn to create in computing courses) then that can more strongly guide the system to scale to more complex programs. We can include these discussions to provide more clarity on this point.  


-------------------------------------
## Complexity of the Synthesis Algorithm
-------------------------------------
Following the reviewers’ observations, we also believe that an ablation study to show the impact of each component of the synthesis algorithm will be valuable. As we were developing the system, we saw improvements with our techniques for each of the three phases of the algorithm: initialization, expansion and ranking. We will implement the variations of our system with naïve versions for each of the three phases (e.g. comparison to randomized decisions, per the reviewers' suggestion) and shall report the precise results. 

-----------------
## Prompt Generation
-----------------
 Prompt generation is a standard approach in using PTMs that helps to guide the PTM as close as possible to the task at hand, and the prompt is usually limited in size (2048 tokens for GPT-3). When using the PTM, prompt generation is only worth considering if we have more training data available than that can fit in the prompt (in our case this was true for the DeepRegex dataset but not for the StackOverflow datasets for both regex and CSS). When there is more data than that can fit, it is still possible to just use a fixed subset of the training data, and the system performs reasonably well but not optimally (we can perform experiments to report those results if deemed important). However, our work here and also other related research (e.g. https://arxiv.org/abs/2101.06804v1) show that one can design more optimal automated techniques for intelligently constructing a prompt from a large dataset, so that the prompt is most relevant for a given query. Note that this is not a manual process for the end user of our final NLX system: they can simply provide ALL of the training data they have available to our NLX system once, and it can store this internally as a configuration parameter. Then when given a new query from the user, our system will construct the prompt dynamically from all the training data it has and send the prompt to GPT-3: if all the training data fits in the prompt then it will send all of it, otherwise it will execute our prompt-generation method to extract the most relevant subset from the training data to dynamically produce the best prompt. Note that this also does not affect our domain-agnostic property: the user has no additional work than to just provide all the training data that they have and our prompt-generation techniques make no assumptions about the domain and only use general notions of word and string similarity of NL descriptions. 

To summarize, prompt generation is an intelligent feature of our overall NLX algorithm that provides more optimal and automated use of GPT, and does not require any additional effort from the user or domain-specific configurations. For the two small StackOverflow datasets we already show a fixed prompt usage with good results, and we can also perform experiments on the third DeepRegex dataset with a fixed static prompt if the reviewers deem it important. We found the performance with static prompts to still be reasonably good but sub-optimal as compared to what can be achieved when using all of the training data that is available.  



----------------
## Related Works
----------------
Thank you for bringing our attention to specific recent related works, and we will include comparisons to each of these works. 

[TransRegex] The TransRegex technique is a very recent work for which we have not yet found an implementation, though we will attempt an empirical comparison if a working implementation can be found. 
In terms of reported results, their best performance on the realistic StackOverflow dataset (StructuredRegex) is 67.4\%, which is very similar (and slightly less) than our 70\% success on StackOverflow scenarios. This gives some general indication that we may have similar performance on the real-world benchmarks. 
In terms of qualitative differences, firstly, TransRegex is designed specifically for Regular expressions only, while our approach is domain-agnostic and not specialized towards a particular language, and we have shown it to be more generally applicable in at least one other domain of CSS. Secondly, the TransRegex technique is based on two distinct phases of first generating a best regex using an NL model, and then an independent examples-based repair technique to repair this best regex. In contrast, our NLX approach more tightly integrates synthesis by using the set of top candidate programs to guide the synthesis at multiple stages (initialization, expansion and ranking). This benefits the synthesis to be biased in multiple ways: (a) to "mix and match" likely components that may not all necessarily occur in the top program and (b) inferring patterns of operator occurrences across the top programs to infer the overall shape of the target program.  
Additionally, many of their contributions are around training of the model to reward syntactically valid regular expressions and to bake in semantic equivalence of regular expressions -- these steps are orthogonal to our work and may even be applied as domain-specific optimizations on the output of GPT-3 to improve the system further.

[CLOSET] The reviewer rightly points out that closed frequent item-set mining is conceptually very similar in that the goal there is also to find frequent sets while also avoiding redundancy by not finding subsets with the same support. As for differences, the work in that area has focused specifically on “association rules” that follow a flat set-based structure, and the main focus has been on efficient scalable algorithms to more efficiently solve the problem at very large scale of large databases. In contrast, a conceptual difference in our case is that the items of interest are not sets but structured AST components, with redundancy coming from the sub-tree rather than subset relation, and secondly, scalability/efficiency of the inference is not the major obstacle in our case as we are working in the order of few hundreds or thousands of components rather than millions of rows in a database. 

[Code generation based on GPT-3]
As mentioned by the reviewers, there has not been much academic research regarding  code generation using large language models, e.g. GPT-3. This is however an evolving scene and we expect various techniques to emerge in near future. Hendrycks et. al. (https://arxiv.org/pdf/2105.09938.pdf) cited by reviewer B offers a large benchmark set for coding tasks (dubbed APPS), that can be used to systematically evaluate the ability of such techniques in using various data-structures and programming techniques. These benchmarks assume a general purpose language (Python) which is currently not what our NLX system is targeting. However, we think APPS is a valuable framework to track advancements in program synthesis research and would be interesting to explore in our future works. 


-----------
#2 CHANGES
-----------
In addition to general improvements to the write up suggested across reviews, we summarize the plan to perform the following additional work items to include in the paper:

- We will perform an ablation study to show the performance of individual components
- We will investigate related works and include them in the discussion, and if possible, perform empirical comparison. 
- We can add results on using a static fixed prompt for the overall system for all datasets. 
- We will conduct experiments to measure quality of the PTM output (comment #2 from reviewer B). We will include statistics of the proportion of components in the GPT outputs that exist in the ground truth program and the proportion that do not.  




----------------------------------------
#3 DETAILED RESPONSES FOR EACH REVIEWER
----------------------------------------

----------------------------------
## Detailed Response to Review #A 
----------------------------------
Q: The motivation for using the rather uncommon terminology of "sorts"?
A: By "sorts", we just mean "types". We used the term "sorts" because the type systems were relatively simple, but we can switch to using "types" instead if that seems clearer. 

Q: Section 3.1 sounds pretty similar to "closed frequent itemset mining" (e.g., see "CLOSET+: searching for the best strategies for mining frequent closed itemsets"), which the paper should discuss.
A: We address this question in the overview section above on related works (see [CLOSET])

Q:Do the authors believe the approach could be generalized to a general-purpose programming language, e.g., Python or Java? If yes, please provide a sketch of how this would be done.
A: See also the above section in overview on claims of being language agnostic. In practice we do not expect to immediately and directly scale to large programs in highly expressive general purpose programming languages such as Python or Java. However, it is an interesting research direction to build upon our ideas here: for instance, we have done initial experiments on small code snippets in C# with promising results, which suggest a compositional approach to multi-modal synthesis may be valuable: instead of just input-output examples, if the user can provide “traces” of examples over some pseudo-code in natural language (similar to “trace tables” students learn to create in computing courses) then that can more strongly guide the system to scale to more complex programs. We can include these discussions to provide more clarity on this point.  

Q:Can you give evidence that all the different parts of the synthesis algorithm contribute to the overall effectiveness?
A:Following the reviewer's observations, we also believe that an ablation study to show the impact of each component of the synthesis algorithm will be valuable. As we were developing the system, we saw improvements with our techniques for each of the three phases of the algorithm: initialization, expansion and ranking. We will implement the variations of our system with naïve versions for each of the three phases (e.g. comparison to randomized decisions, per the reviewers' suggestion) and shall report the precise results. 

Q:How does your work relate to TransRegex (ICSE'21)?
A: Thank you for pointing this out and we address this in the overview section above on related works (see [TransRegex])



----------------------------------
## Detailed Response to Review #B
----------------------------------

Q: [comment #2]  measure quality of GPT output 
A: Yes, for more insight on the quality of the PTM outputs, we will include statistics of the proportion of components in the GPT outputs that exist in the Ground truth program and the proportion that do not. 

Q: [comment #4] Sec 4 bothers me.  Why do we need to provide similar questions as a prompt?  Is this realistic in a domain-agnostic approach?  Also, if the prompt was populated by the same 3-4 canned examples, followed by the specific question, how much does the overall effectiveness drop ?  (See #7 below also.)
A: Section 4 describes an "optimization" step . Even without it (and with picking the same-4 canned examples) our approach works, with a slight drop in accuracy (more discussion below). Section 4 is realistic in a domain-agnostic approach as it can be used whenever there are examples available, and it works solely at the level of string similarity (no domain-specificity here).

Prompt generation is a standard approach in using PTMs that helps to guide the PTM as close as possible to the task at hand, and the prompt is usually limited in size (2048 tokens for GPT-3). When using the PTM, prompt generation is only worth considering if we have more training data available than that can fit in the prompt (in our case this was true for the DeepRegex dataset but not for the StackOverflow datasets for both regex and CSS). When there is more data than that can fit, it is still possible to just use a fixed subset of the training data, and the system performs reasonably well but not optimally (we can perform experiments to report those results if deemed important). However, our work here and also other related research (e.g. https://arxiv.org/pdf/2102.09690.pdf) show that one can design more optimal automated techniques for intelligently constructing a prompt from a large dataset, so that the prompt is most relevant for a given query. Note that this is not a manual process for the end user of our final NLX system: they can simply provide ALL of the training data they have available to our NLX system once, and it can store this internally as a configuration parameter. Then when given a new query from the user, our system will construct the prompt dynamically from all the training data it has and send the prompt to GPT-3: if all the training data fits in the prompt then it will send all of it, otherwise it will execute our prompt-generation method to extract the most relevant subset from the training data to dynamically produce the best prompt. Note that this also does not affect our domain-agnostic property: the user has no additional work than to just provide all the training data that they have and our prompt-generation techniques make no assumptions about the domain and only use general notions of word and string similarity of NL descriptions. 

So to summarize, prompt generation is an intelligent feature of our overall NLX algorithm that provides more optimal and automated use of GPT, and does not require any additional effort from the user or domain-specific configurations. For the two small StackOverflow datasets we already show a fixed prompt usage with good results, and we can also perform experiments on the third DeepRegex dataset with a fixed static prompt if the reviewer deems it important.  


Q: [comment #5] In Sec 5.1.2 I am not sure why this is an argument to support domain-agnostic approach.  This is more a problem with Regel in that it might be somewhat overfitted to the DeepRegex suite. 
A: Fully agreed and we will reword - we were not intending to claim that we perform better because of being domain-agnostic, but instead just pointing out that our approach performs well despite being domain-agnostic, as opposed to the specialized Regel system.


Q: [comment #5]  Why Regel did not do so well on the Stack Overflow suite? Was sketch generation the issue or was the subsequent phase the issue?
A: Regel failed to generate the skectch for 1 (out of 20) case. The rest of failed cases were due to time-outs from the SMT solver (we do not know if this was due to low quality of sketches or for other reasons). 

Q: [comment #7] I am puzzled why the BFS performance is pretty good in the CSS case study but not so good in the Regex case study.   I would have expected BFS to do not so poorly across the board, because it does pick its ingredients from PTM predictions (at least one time.).   I am not sure how the authors could inspect this further, but I wonder if somehow picking the right prompt is giving NLX an unfair advantage in the Regex case study.
A: The main reason for better BFS performance for CSS is that the grammar was relatively simpler for CSS, and the target programs are also relatively smaller in terms of AST size/complexity (every literal character in a regex uses a concatenation operator while CSS selectors often contain usually around 4 or 5 logical filtering constraints). Picking the prompt will not give NLX an unfair advantage because both NLX and BFS were provided the same output from GPT that was obtained with the same best prompt that was sent to GPT. The only differences between NLX and BFS are in how they handle the subsequent phases of synthesis when given the same GPT results.




----------------------------------
## Detailed Response to Review #C
----------------------------------
Q: Is the prompt in Figure 5 the exact query used to get the set of plausible programs?
A: Yes, it is the prompt used for the completion shown below. For other completion tasks, the actual (NL,Regex)-pairs shown in Figure 5 may be replaced by other pairs depending on their relevance to the user's NL query.

Q: Why does the similarity check actually hurt for $R_{TM}$?  Why is that outcome worse than random?
A: At a high level, the reason is that a random prompt is better than a misleading prompt. Token matching (TM) can potentially select Q&A pairs that may mislead GPT3, and forcing diversity (similar check) can exacerbate this effect: TM tends to pick questions that have the same Stop words (words that are common but do not contribute much to semantics), and by forcing diversity, we pick more such questions that have very different semantics. In short, R-{TM} with similary check can be worse than random because random will not bias GPT3 as much as the "similar looking questions" whose "answers are completely different from the ground truth" selected by R-{TM}.


Q: What other plausible ways might the tool extract guidance for rankings?
A: We did experiments with different notions of similarity between programs (including various tree or string distance measures). In the paper we presented the string similarity measures which yielded the best results. It is an intriguing research question to define and systematically evaluate such notions of similarity, which we had deemed outside the scope of the paper, but we can include more discussion on that if the reviewer feels it is important. 

Q: Why was the prompt generation approach not evaluated further? For instance, why was it not compared against using a single hand-crafted prompt for all tasks in a given domain?
A: We will add a comparison to a fixed hand-crafted prompt in the revision. Based on our preliminary experiments conducted before designing our prompt generation approach, a single static prompt does not perform as well as any of the approaches we presented in the paper.

Q:Section 5 also increases my concern about the sensitivity to prompt generation.  If the DeepRegex test (respectively, the StackOverflow test) pulled on training data from only the DeepRegex dataset (respectively, the StackOverflow dataset), then it’s not just making one prompt/prompt template for a given domain but for *slices* of each given domain.  This makes it much harder than the introduction suggests to generalize this approach, since we seem to still need a small- to medium-sized body of input-output examples to do “training” (prompt generation), even though we’re using pre-trained models.  
A: To clarify, in our experiments for the regex domain, we only performed prompt generation for the DeepRegex dataset as there was significant training data available. For the StackOverflow dataset we just used a fixed set of 5 cases for the prompt because the dataset was very small. Hence prompt-generation is not a necessity for our approach but only an automated optimization when large amount of training data is available (how to use it best if available). If deemed important, we can report results with a fixed static prompt for DeepRegex also, which are sub-optimal but not severely worse.





==> Reviews/Kia-draft.tex <==
We thank the reviewing committee for their detailed reviews and insightful comments. We will incorporate all suggestions for improvement of the paper in the future versions.



-----------------------------------------------
Claims of being language-agnostic (All Reviews)
-----------------------------------------------
We agree that we may have stressed the generality of our approach perhaps too strongly and we will clarify its scope and expected limitations. Our goal is not to claim that our approach can be directly applied to any arbitrary language, but only that it is not specialized to one particular language, and we support this by showing its applicability and benefits in two very different programming domains. We discuss some expected limitations in points C and D in section 7. In particular, our approach does rely on a well-defined notion of input-output examples that the user can easily provide, and evaluation of sub-expressions on the inputs should produce well-defined outputs that can be compared during synthesis (using notions  of semantic equivalence). We do not assume that the inputs of a program and the parse tree of the program follow the same hierarchical decomposition (e.g. in CSS there is no such direct correspondence), but it is true that our approach is more effective when sub-expressions produce meaningful semantic values in a compositional manner. We have discussed expected improvements to handle other domains such as Pandas, and in practice we do not expect to immediately scale to large programs in highly expressive general purpose programming languages such as Python or Java. However, it is an interesting research direction to build upon our ideas here: for instance, we have done initial experiments on small code snippets in C# with promising results, which suggest a compositional approach to multi-modal synthesis may be valuable: instead of just input-output examples, if the user can provide “traces” of examples over some pseudo-code in natural language then that can more strongly guide the system to scale to more complex programs - similar to “trace tables” students learn to create in computing courses. We can include these discussions to provide more clarity on this point.  


---------------------------------------------------
Complexity of the Synthesis Algorithm (All Reviews)
---------------------------------------------------


Following the reviewers’ observations, we also believe that an ablation study to show the impact of each of these components will be valuable. As we were developing the system, we saw improvements with our techniques for each of the three phases of the algorithm: initialization, expansion and ranking. We will implement the variations of our system with naïve versions for each of the three phases (e.g. comparison to randomized decisions, per the reviewers' suggestion) and shall report the precise results. 






--------------------------------
Prompt Generation (All reviews )
--------------------------------
Following the recommendations from the designers of the GPT-3 system [cite], we designed our synthesizer to first “teach” the PTM about the domain of the synthesis tasks to be queried. This approach is known as few-shot learning, which enables the NLX system to define the context for each task using only a handful of examples — unlike generic training approaches (e.g. REGEL) where the size of the training set is usually orders of magnitudes larger.  

For each benchmark-set we used a small and randomly chosen subset of the cases to generate the prompts for the queries from that set. This is a standard approach and is also used in the baseline system Regel.  Given this set of question-answer pairs, in section 4, we try to further improve the “quality” of the prompts. As a proxy for the notion of quality for the prompts, we measured the number of cases where the PTM’s output is semantically equivalent to the ground-truth. 

We observed that the GPT-3 system was capable of providing necessary constructs to synthesize the target program — even when a generic prompt was used for all tasks, which was not fine-tuned for each query.  Hence, we do not believe that the overall performance of NLX system is crucially dependent on the optimizations provided in section 4 — this is specially true for the StackOverflow data set where the test-cases are drastically different from each other.  

We agree with the reviewers that it will be interesting to study the impact of different prompts on the overall performance of the NLX system. We plan to conduct further experiments with this regard and will present our findings in the next versions of the paper. 



----------------------------
Related Works (All reviews )
----------------------------
Thank you for bringing our attention to specific recent related works, and we will include comparisons to each of these works. 

[TransRegex] The TransRegex technique is a very recent work for which we have not yet found an implementation, though we will attempt an empirical comparison if a working implementation can be found. In terms of reported results, their best performance on the realistic StackOverflow dataset (StructuredRegex) is 67.4\%, which is very similar (and slightly less) than our 70\% success on StackOverflow scenarios. This gives some general indication that we may have similar performance on the real-world benchmarks. In terms of qualitative differences, firstly, TransRegex is designed specifically for Regular expressions only, while our approach is domain-agnostic and not specialized towards a particular language, and we have shown it to be more generally applicable in at least one other domain of CSS. Secondly, the TransRegex technique is based on two distinct phases of first generating a best regex using an NL model, and then a separate examples-based repair technique to repair this best regex. In contrast, our NLX approach more tightly integrates synthesis by using the set of top candidate programs to guide the synthesis at multiple stages (initialization, expansion and ranking). This benefits the synthesis bias in multiple ways: (a) to "mix and match" likely components that may not all necessarily occur in the top program (b) inferring patterns of operator occurrences across the top programs to infer the overall shape of the target program.  

Additionally, many of their contributions are around training of the model to reward syntactically valid regular expressions and to bake in semantic equivalence of regular expressions -- these steps are orthogonal to our work and may even be applied as domain-specific optimizations on the output of GPT-3 to improve the system further.


[CLOSET] The reviewer rightly points out that closed frequent itemset mining is conceptually very similar in that the goal there is also to find frequent sets while also avoiding redundancy by not finding subsets with the same support. As for differences, the work in that area has focused specifically on “association rules” that follow a flat set-based structure, and the main focus has been on efficient scalable algorithms to more efficiently solve the problem at very large scale of large databases. In contrast, a conceptual difference in our case is that the items of interest are not sets but structured AST components, with redundancy coming from the sub-tree rather than subset relation, and secondly, scalability/efficiency of the inference is not the major obstacle in our case as we are working in the order of few hundreds or thousands of components rather than millions of rows in a database. 

[Code generation based on GPT-3]
@Kia please look at this paper cited by the reviewer https://arxiv.org/pdf/2105.09938.pdf ?
and briefly comment on it and any other related works. 


%In particular, our work has a few fundamental differences with the TransRegex (ICSE’21) paper. Although both approaches utilize an NL model to produce candidate  expressions from the NL descriptions, the NLX system is designed to synthesize the ground-truth using the set of all candidates, while TransRegex attempts to repair only the top candidate. This means that the NLX system can utilize the stochastic nature of the PTM models — by allowing it to (a) “mix-and-match” components from multiple candidates and (b) to guess the overall shape of the ground-truth and use it to guide the search. 

%On the other hand, the TransRegex system (similar to REGEL) performs a search over the space of expressions which are structurally similar to the candidate expressions. This approach however will not work well if the target expression is not within a fixed neighborhood of the output. Theoretically, our approach should be more biased towards components and operators that are more likely to be used in the ground-truth. 

%Additionally, the TransRegex approach is tightly entangled with the domain of regular expressions. In particular, their abstract representation of programs is designed according the particular semantics of regular expressions (e.g. <S> replaces concrete expressions such as .*..* -- this helps reduce the space of neighbor expressions drastically). It is not immediately clear how this approach would be applied in other domains.  Furthermore, TransRegex attempts to bake-in the semantic equivalence of regular expressions into the model as a mechanism to improve the NL-to-Regex performance.

%Finally, the best performance reported for TransRegex on the most realistic dataset (StructuredRegex, which is based on StackOverflow questions) is 67.4\%, that is very similar to our 70\% success on StackOverflow scenarios. This indicates that generally both approaches may have similar performance on the real-world benchmarks. 

%We were unable to find a link to the TransRegex implementation, but will try to access it and conduct further experiments to compare both approaches empirically. In any case, we will include a detailed discussion regarding their work in the related works section of the paper.


@Kia - do we want to touch on here some of the comments about how the "prompt generation" also prohibits this from being an entirely "domain agnostic" system, as the few-shot learning of GPT-3 does require some examples to work effectively (although, not many)
Mohammad: I dont think it makes it less domain-agnostic, because user can just provide those examples as parameter to our system. 


----------------------------------
### Detailed Response to Review #A
----------------------------------
## The motivation for using the rather uncommon terminology of "sorts"?




----------------------------------
### Detailed Response to Review #B
----------------------------------
## I am puzzled why the BFS performance is pretty good in the CSS case study but not so good in the Regex case study.





## Why Regel did not do so well on the Stack Overflow suite: was sketch generation the issue or was the subsequent phase the issue?






----------------------------------
### Detailed Response to Review #C
----------------------------------


## Is the prompt in Figure 5 the exact query used to get the set of plausible programs?


## Why does the similarity check actually hurt for $R_{TM}$?  Why is that outcome worse than random?



## What other plausible ways might the tool extract guidance for rankings?



## Why was the prompt generation approach not evaluated further? For instance, why was it not compared against using a single hand-crafted prompt for all tasks in a given domain?

==> Reviews/Mohammad-draft.tex <==
We thank the reviewing committee for their detailed reviews and insightful comments. We will incorporate all suggestions for improvement of the paper in the future versions.



-----------------------------------------------
Claims of being language-agnostic (All Reviews)
-----------------------------------------------

We have clarified our implicit assumptions about the DSLs under consideration in Section 7. \COMMENT{Mohammad: remove this, i dont think it clarifies the DSL assumptions or answers the reviewer's concern - may seem redundant and careless}

We do not currently have any concrete evidence that our approach would generalize to arbitrary general-purpose programming languages.

However, even within general-purpose languages (e.g. java) arbitrary DSLs may be defined for particular problems  which our approach may work on. 

It was not our goal to demonstrate this as a core contribution, but more that the ideas can be applicable accroass multiple domains. and our approach is not fine-tuned for any particular use-case. 

It is not immediately clear how our ideas can be applied on languages which are very expressive. We leave this for future works. 

We can design a DSL on top of general-purpose languages for specific problem domains. This requires understanding the specific property of the languages that this will work on.

The claims that the approach as it stands is applicable to any language was not our intent. 

We tried to emphasize on the fact that our approach does not fundamentally rely on any domain-specific techniques.

The main goal of this paper is to formally introduce pre-trained language models as a viable solution for guiding program synthesis approaches. 

Restricted DSLs are necessary for our approach. However, for particular domains we may be able to define the DSL on top of the general-purpose language. 

It is an intriguing research question to formalize these constraints, which we leave for future works


---------------------------------------------------
Complexity of the Synthesis Algorithm (All Reviews)
---------------------------------------------------
As we were developing the system we identified improvements in different aspects of the algorithm -- which guided the final design of the NLX algorithm. It is indeed interesting to identify the impact of each component on the performance of the overall approach. We will design an ablation study and conduct further experiments to gauge the impact of each component in the NLX algorithm. 


The space of valid programs is huge, and we have designed these components to prune the space and guide the search. 



We will define various baselines (e.g. comparison to randomized decisions, per the reviewers' suggestion) of the NLX algorithm and present the findings in the next versions of the paper. 







--------------------------------
Prompt Generation (All reviews )
--------------------------------
Our synthesis algorithm is on top of a few-shot learning technique which "teaches" the model about the task in hand. Per reviewer's observation, the performance of the overall approach critically depends on this step.

In the few-shot learning approach, the model is given a small context containing a few examples of the task in hand and at the end is given a new task to respond to. This is how we can "teach" the PTM about problem domain. While effectively training a specialized model requires a huge number of examples and manual effort, PTMS -- due to their design features -- allow developers to steer the results into a particular domain by defining a context. The prompt generation is a relatively easier and less costly task. In section 4 we present a formative study for this process which explains how different approaches for generating the prompt will impact the "quality" of the final output. We used the number of correct outputs as a proxy for the quality of the prompt and use the best setup for our final evaluation of NLX. 



In section 4 we present our approach in detail. In particular, we explain the "context" of the learner is constructed from a set of 


While the size (number of question-answer pairs) of the prompt was the same for all cases, the prompt was generated for each case individually, according to the procedure explained in section 4. 

We did use randomly chosen cases from each benchmark set to create the prompt - this is a standard approach is also used in the baseline system Regel. We were able to construct the prompt using a small number of examples (5 to 10) while the number of examples needed for training specialized models is much larger (hunderds or thousands)


It is an intriguing research question to define other measures of quality (e.g. number of use-less components) for the output of the PTM with respect to a cost model that effectively captures the synthesizer's behaviors. 


----------------------------
Related Works (All reviews )
----------------------------
We were not aware of the related works cited by the reviewers, at the time of submission. We will provide a detailed comparison to these works in the next version of the paper. 

The main difference between NLX and TransRegex is that the former is a synthesizer while the latter is inherently a repair mechanism. There are similarities between their approaches, specially regarding the use of an NLP model to collect a set of broken expressions. In particular, the synthesis approach has the advantage of being able to mix-and-match components from multiple faulty expressions. Our approach also extracts  information the target program from the set of expressions generated by the PTM (e.g. the distribution of each operator is determined from the set of expressions, not any single expression)
Their repair is limited to minor changes in the 


Also, the way they use language model is very different than our approach. In particular, they introduce a 2-phase algorithm to achieve high performance from the NL model (while in our approach the PTM is mostly treated as a black box)

This approach - similar to REGEL - performs an efficient search over the space of expressions which are structurally similar to the expression generated by the PTM. This approach however will not work well if the target expression is not close to the output.


This approach is composed of two main parts: the NLP-based regex synthesis and example-guided regex repair. 


Their approach is to transform the NL model's concrete expression into an abstract expression whose neighbourhood of similar abstract expressions is explored using a set of subtle rewrite rules -- e.g. the rule which adjusts the position of a quantifier in an expression. There are two aspects of this approach which are tightly entangled with the domain of regular expressions; in particular, 
their abstract representation of expressions is designed around the semantics of regular expressions (e.g. <S> replaces concrete expressions such as .*..* -- this helps reduce the space of neighbor expressions drastically.) It is not immediately clear how this approach would be applied on other domains. 
Additionally, their contributions mostly revolves around the training of their model, which is done in a way to reward syntactically valid regular expressions and to bake in semantic equivalence of regular expressions -- as a mechanism to improve the NL-to-Regex performance. Using another model to transform syntactically invalid regular expressions to valid ones, they are able to get 100\% syntactically correct regular expressions from NL description -- these steps are orthogonal to our work and can be even applied on the output of GPT-3 to get rid of syntactically invalid programs. 

\COMMENT{Mohammad: this seems too detailed and I dont think looks relevant - even if it is orthogonal the main question is if/how/why their approach is better o worse}


Transregex comparision points:
o	They are Domain-specific, we are domain-agnostic
o	They use NLP + repair. They repair a single top regex, whereas we take the set of top ranked programs and use commonly occurring components from all these programs – this theoretically gives more bias towards components that are more likely to be used. 
o	Their best performance on the realistic dataset (StructuredRegex) which is based on StackOverflow questions is 67.4%, which is very similar to our 70% success on StackOverflow scenarios. So this indicates that generally we may have similar performance on the real-world benchmarks.
o	We cannot find a link to their implementation, but will try to see if we can access it, otherwise include it in our discussion. 



----------------------------------
### Detailed Response to Review #A
----------------------------------






----------------------------------
### Detailed Response to Review #B
----------------------------------



----------------------------------
### Detailed Response to Review #C
----------------------------------






==> Reviews/extracted_reviews.tex <==

(1) Claims of being language-agnostic:
    (1.1)(#A) The paper repeatedly claims that the approach is language-agnostic and should work well for arbitrary DSLs. While the two implementations for regexes and CSS support partially this argument, I'm wondering what implicit assumptions the authors make about the DSLs. 
    For example, the notion of semantics described on page 6 seems to assume that the inputs of a program and the parse tree of the program follow the same hierarchical decomposition. Do the authors believe the approach could be generalized to a general-purpose programming language, e.g., Python or Java? If yes, please provide a sketch of how this would be done.
    
    //we agree that it has it's limitations, shows generality, two domains, ideas valid across domains, say something about which domains it will and won't work in, e.g languages like c# and java
    //we don't expect it to be applicable to languages which are very expressive, restriction of DSL is necessary.
    //Possibly design a DSL ontop of those more expressive languages for specific problem solvings, crystallize the specific property of the languages that this will work on
    //point them to section 7 - procedure multi step multi optimised, some of the optimisations are not possible for more general synthesis, e.g execution of partial sub-programs. just because some steps are not possible doesn't mean the entire approach is not useful. 
    //Does the technology scale without these optimisations?
    
    (1.2)(#B)  I felt that the domain-agnostic success of this paper is a bit oversold.  We have seen results on just two domains, and have seen that the idea does not work on a different domain (Sec 7.)
    
    // wasn't really our goal to demonstrate this as a core contribution, but more that the ideas can be applicable. - 1 more example ? cannot promise another domain
    
------------------------------------------------------------------------------------------------------------------------------
2) Unclear if complexity of the approach is needed (ablation study):
    (2.1)(#A) The approach uses the candidate answers provided by the model to influence the component-based synthesis in various way. Overall, this yields a pretty complex approach, and it's not clear if all this complexity is needed. It would be great to see an ablation study that omits parts of the guidance (and replaces it with, e.g., a purely random alternative). E.g., what happens when the initialization of components randomly samples from the candidate answers, when the pruning doesn't check which subterms are semantically equivalent, or when the synthesized programs are ranked randomly? Can you give evidence that all the different parts of the synthesis algorithm contribute to the overall effectiveness?
    
    // as we were developing the system we found the improvements in different parts of the algorithm, would've been good to have those results but we don't have them. as we found them during the development and don't have exact results to report right now, system is not designed in a way to give us these results quickly
    // report in the paper final version some random baseline, even using some cheaper model
    // we should do this ablation study, some of the aspects are not hugely compelling with only small improvements
    
    (2.2)(#C) I would have loved to see variants on the BFS baseline.  I.e., NLX-Reg without initialization, without expansion, without ranking. This would help to understand whether *all* of these techniques were really required.  I’m particularly interested in whether expansion really improved performance, but I think all three would offer interesting insights.
    
    // see above

------------------------------------------------------------------------------------------------------------------------------
(3) Related Works:
    (3.1)(#A) The TransRegex technique presented at ICSE'21 (but available on https://arxiv.org/abs/2012.15489 since 12/2020) also proposed multi-modal synthesis of regular expressions through a combination of learning-based prediction and example-based refinement of predicted candidate regexs. How does the proposed approach related to TransRegex? It would be great to see an empirical comparison with this technique.
    
    // outline the differences of the approaches, say we will expand in the paper
    // read the paper in a bit more detail, develop our own understanding and insight
    // another specialised system for regex. state of the art WAS regel, but these are solving a more specialised problem, rather than the more general approach we are taking
    // see if we can run their system
    // look at the technical details, even if we don't compare experimentally, if we are technically different that may be enough
    // we use fewer examples, they need 10 positive 10 negative, justification for lower precision potenitally
    // we will try to find this tool and run an evaluation. but in terms of theory we are different because of X Y Z
    //they use encoder-decoder, then repairs
    //they use a set of repair techniques, some rewriting rules 
    //second part of the repair is the most interesting comparison, sell the generality 
    //relative completeness? we use only components of GPT-3
    //why didn't they re-run regel, they just applied their tool on the same dataset
    //make a claim they didn't compare on realistic examples from stack overflow, comment on their datasets
    //does structuredRegex contain examples from stack overflow?
    // about the comparison against TransRegex, Section 4 is also a contribution of our approach. We propose to use a general PTM instead of a specific transformer model for that domain, which would require much more data. So, I agree with Dan. They could not use GPT-3 out-of-the-box without the few shot learning approach we proposed 
    
    3.2)(#A) Section 3.1 sounds pretty similar to "closed frequent itemset mining" (e.g., see "CLOSET+: searching for the best strategies for mining frequent closed itemsets"), which the paper should discuss.
    
    // add citation and discuss how this relates to our initialization of components/maximal components
    
    3.3)(#B) Granted that GPT-3 is very new, aren’t there other papers, even informal, that should be mentioned in the Related Work in the space of code generation based on GPT-3? What about https://arxiv.org/pdf/2105.09938.pdf ?
    
    // look at the paper in the related work, a section about code generation from PTMs, need to read this particular paper

------------------------------------------------------------------------------------------------------------------------------

(4) Prompt Generation:
    (4.1)(#A)  Section 4 describes how to choose the best question-answer pairs to include in the prompt for a specific question q*, but then Sections 5.1.1 and 5.2 mention that a fixed set of question-answer pairs is used for the evaluation. What am I missing here?
    
    // elaborate on how even though fixed number were used, the examples contained within it do change
    
    (4.2)(#B) The act of prompting the GPT-3 model using very-related questions might be an unfair advantage, depending on the domain we are using this system for, and it may be an unreasonable way of using the system. Why do we need to provide similar questions as a prompt?  Is this realistic in a domain-agnostic approach?  Also, if the prompt was populated by the same 3-4 canned examples, followed by the specific question, how much does the overall effectiveness drop?
    
    // the technique does require examples. but the technique itself will work cross domain, so while we may need to "retrain" on other datasets. 
    // be careful answering this one, we have to say this is essentially what few-shot learning is
    // results are influenced by the dynamic prompt, our study shows if we used random.
    
    (4.3)(#C) How dependent is the system on how ‘similar’ (quotes since I provide no definition for similarity here) the training-time NL queries are to the users’ plausibly quite different NL queries?  It seems plausible that this could work well for a suite of NL prompts with similar style, pulled together by the research team (and used for the initial few-shot learning query), but fail to work nicely for users’ more diverse prompts. I’m not worried that the synthesis part of the process will fail to explore the space of programs--we’re worried that the machine learning part of the process will fail to provide the necessary constructs. 
    
    // do we need to provide final results with and without these techniques
    // "how much it depends on this setup"
    
    (4.4)(#C) Is the prompt in Figure 5 the exact query used to get the set of plausible programs?  Constructing this query could be one of the most sensitive parts of this process.  (Making the domain-specific query could also make it hard to extend the work to additional domains, despite the paper’s claims about domain-independence.)  This is ultimately explained in Sec 4, but it would help to see more detail earlier.
    
    // no it is not
    // this is not the exact input, the content of the NL : {1} and Regex: {2} varies
    // clarify what we can do in the next version of the paper
    
    (4.5)(#C) "If the distance is less than a threshold t then the answers are considered too close and the question-answer pair is discarded. This is to ensure that the PTM is not biased toward a particular group of tasks and does not produce sub-optimal results."  
    How did the authors realize/observe this in the first place?  Very interesting.  Why does the similarity check actually hurt for $R_{TM}$?  Why is that outcome worse than random?  Great discussion in 4.1.2, and I’d love to see more on this topic.
    
    // when we were using the deepregex set for training, the first N results would all the regex with varying natural language due to the size of the training set. With very little variance in the regex provided the results suffered greatly. 
    // run it for dynamic context again with similarity metric, there is an unanswered question here
    
    (#C) If the DeepRegex test (respectively, the StackOverflow test) pulled on training data from only the DeepRegex dataset (respectively, the StackOverflow dataset), then it’s not just making one prompt/prompt template for a given domain but for *slices* of each given domain.  This makes it much harder than the introduction suggests to generalize this approach, since we seem to still need a small  body of input-output examples to do "training" (prompt generation), even though we’re using pre-trained models.  It’s reasonable to promote the domain independence in comparison to a tool like Regel, but the introduction overpromises a bit.
    
    // we need fewer examples than any model that would be trained to do it would need, more of a question we should revisit on generality
    //about the comparison against TransRegex, Section 4 is also a contribution of our approach. We propose to use a general PTM instead of a specific transformer model for that domain, which would require much more data. So, I agree with Dan. They could not use GPT-3 out-of-the-box without the few shot learning approach we proposed 
    
    
------------------------------------------------------------------------------------------------------------------------------
(5) Presentation-related comments:
    (5.1)(#A) The motivation for using the rather uncommon terminology of "sorts" for describing the DSL isn't clear. E.g., Figure 2a looks like definition of tokens and parse trees. How do "sorts" related to non-terminals and to types?
    
    // Mohammad has the same question, why use sorts vs types
    // discussed this with Ashish at some point, we can use either one
    
    (5.2)(#B) In Sec 5.1.2 I am not sure why this is an argument to support domain-agnostic approach.  This is more a problem with Regel in that it might be somewhat overfitted to the DeepRegex suite. 
    
    // this particular issue has nothing to do with the domain agnostic-ness of our approach
    
    (5.3)(#B) It is not reported why Regel did not do so well on the Stack Overflow suite: was sketch generation the issue or was the subsequent phase the issue?
    
    //no, sketch generation failed only one case, the rest were failing in the synthesis step
------------------------------------------------------------------------------------------------------------------------------    
(6) Additional Evaluations 
    (6.1)(#B) I would have liked to see some more empirical validation on how well the PTM predictions contain "good" ingredients for the eventual solution, and do not contain useless ingredients.  This is not a weakness of the paper, but given the number of DSL-based papers in synthesis, and already some successes, I would have liked to see how well this kind of approach (that uses GPT-3) can work with more general coding tasks.
    
    //if we could measure how good the output of GPT is directly before synthesis. how many good ingredients vs bad ingredients. 
    //pose the problem via final ground truth from gpt candidates, what percentage of the ground truth exists in any of the GPT candidates
    // somewhat different to actually solving the task
    // promise this
 
    (6.2)(#B) I am puzzled why the BFS performance is pretty good in the CSS case study but not so good in the Regex case study.   I would have expected BFS to do not so poorly across the board, because it does pick its ingredients from PTM predictions.  I am not sure how the authors could inspect this further, but I wonder if somehow picking the right prompt is giving NLX an unfair advantage in the Regex case study.
    
    //prompt use is a contribution rather than an unfair advantage
    //proper prompt reduce number of bad candidates?
    //doing better in CSS as the search space is smaller, number of components is somewhat fewer.
    
    (6.3)(#B) Many enumerative synthesis papers employ some sort of prioritization strategy (e.g. using weights in TF-Coder paper LINK).  Here the prioritization is derived from the output of the PTM model.   This last assumption should be validated independently because this seems to be the essential nugget that can be leveraged in follow up research on this topic. (This is notwithstanding the issues already found in Sec 7.). An ideal PTM output would contain a small number of terms and operators that are needed in the solution.  How far from ideal did we get for various problems ?
    
    //some better understanding of the GPT output. we took them directly
    //somewhat orthogonal
    //want more work on getting the best output from the PTM?
    

    (6.5)(#C) Why was the prompt generation approach not evaluated further?  (That is, further than in 4.1.)  For instance, why was it not compared against using a single hand-crafted prompt for all tasks in a given domain?
    
    // the static results could be useful here
    // 
    
    (6.6)(#C) Overall, I would have loved to see more variants explored.  E.g., what other plausible ways might the tool extract guidance for rankings?  Incorporating string similarity is interesting, but what are other points in this space?
    
    // we never tried tree-edit-distance, different measures of similarity, we can add a discussion for this.
    // don't promise experiments, best we can get without going into detail?
    // domain specific optimisations knowing knowledge of the operators
    // we did not include the domain-specific to keep the message simple 
    
------------------------------------------------------------------------------------------------------------------------------    
(7) Misc:
    (7.1)(#B) Given additional positive and negative examples, couldn't the synthesizer get more specific information that it can use to guide the search (e.g. additional pruning along unpromising paths) 
    
    // we do use examples to guide the search.
    
------------------------------------------------------------------------------------------------------------------------------

==> Reviews/original_reviews.tex <==
OOPSLA 2021 Paper #410 Reviews and Comments
===========================================================================
Paper #410 Multi-modal Program Inference: a Marriage of Pre-trained
Language Models and Component-based Synthesis


Review #410A
===========================================================================

Overall merit
-------------
3. Weak accept

Review confidence
-----------------
2. Medium

Paper summary
-------------
This paper describes a program synthesis technique guided by a general-purpose, neural, question-answering model. Given a natural language description of the code to synthesize, the first step is query the model. For this purpose, the authors query a GPT-3 model with a short context description and a few examples of question-answer pairs (few-shot learning). Next, the answers provided by the model are used to guide several aspects of a component-based synthesis algorithm: what components to initialize the search with, which operators to use to expand given components into new code, and what examples to prune from the search. To answer these questions, the paper proposes algorithms based on the frequency of components and operators in the answers offered by the model. The work is evaluated with two datasets of regular expressions, comparing with the existing Regel approach, and with a small dataset of CSS selectors.

Strengths and Weaknesses
------------------------
Strengths:
* Interesting combination of general-purpose, pre-trained model and component-based synthesis
* Empirical evidence for increased accuracy over the state-of-the-art
* Well-written

Weaknesses:
* Claims of being language-agnostic aren't fully backed up by evidence
* Complex approach, but no ablation study to show that complexity is needed
* Strongly related ICSE'21 paper not cited

Comments for author
-------------------
This is an interesting paper. In particular, I like the overall idea of combining a GPT-3 model, which is general purpose and not aimed at all at program synthesis, with a component-based synthesis algorithm. Intuitively, the combination of these two approaches nicely uses their respective strengths. I also like most parts of the evaluation, which shows benefits over a sate-of-the-art approach for regular expression synthesis. Finally, the paper is well-written, making good use of examples while describing the approach precisely and thoroughly.

Besides these positives, there are three concerns that limit my enthusiasm:

1) Overclaiming of generality:

The paper repeatedly claims that the approach is language-agnostic and should work well for arbitrary DSLs. While the two implementations for regexes and CSS support partially this argument, I'm wondering what implicit assumptions the authors make about the DSLs. For example, the notion of semantics described on page 6 seems to assume that the inputs of a program and the parse tree of the program follow the same hierarchical decomposition. Do the authors believe the approach could be generalized to a general-purpose programming language, e.g., Python or Java?

2) Unclear if complexity of the approach is needed

The approach uses the candidate answers provided by the model to influence the component-based synthesis in various way. Overall, this yields a pretty complex approach, and it's not clear if all this complexity is needed. It would be great to see an ablation study that omits parts of the guidance (and replaces it with, e.g., a purely random alternative). E.g., what happens when the initialization of components randomly samples from the candidate answers, when the pruning doesn't check which subterms are semantically equivalent, or when the synthesized programs are ranked randomly?

3) No discussion of TransRegex (ICSE'21)

The TransRegex technique presented at ICSE'21 (but available on https://arxiv.org/abs/2012.15489 since 12/2020) also proposed multi-modal synthesis of regular expressions through a combination of learning-based prediction and example-based refinement of predicted candidate regexs. How does the proposed approach related to TransRegex? It would be great to see an empirical comparison with this technique.

Other comments:
 * One aspect of the experiment setup is unclear: Section 4 describes how to choose the best question-answer pairs to include in the prompt for a specific question q*, but then Sections 5.1.1 and 5.2 mention that a fixed set of question-answer pairs is used for the evaluation. What am I missing here?

Some mostly presentation-related suggestions:
 * The motivation for using the rather uncommon terminology of "sorts" for describing the DSL isn't clear. E.g., Figure 2a looks like definition of tokens and parse trees. How do "sorts" related to non-terminals and to types?
 * Section 3.1 sounds pretty similar to "closed frequent itemset mining" (e.g., see "CLOSET+: searching for the best strategies for mining frequent closed itemsets"), which the paper should discuss.
 * asses --> assess (at least two times)
 * that not supported --> that is not supported

Questions for authors’ response
---------------------------------
Do the authors believe the approach could be generalized to a general-purpose programming language, e.g., Python or Java? If yes, please provide a sketch of how this would be done.

Can you give evidence that all the different parts of the synthesis algorithm contribute to the overall effectiveness?

How does your work relate to TransRegex (ICSE'21)?



Review #410B
===========================================================================

Overall merit
-------------
4. Accept

Review confidence
-----------------
3. High

Paper summary
-------------
This paper concerns synthesis of regular expressions starting from a natural language description of what a programmer desires, as well as a few input-output examples to clarify the desired intent.  (The paper claims that it is domain agnostic.) Since natural language is generally ambiguous, no automated code generation from NL has been shown to work with good reliability.  At the same time, providing examples only is tedious, and therefore it is often desired to use examples only as a way to compensate for the ambiguity of natural languages descriptions.  This kind of synthesis is called multi-modal synthesis.  

The proposed approach is to first use a GPT-3 style pre-trained generative model (PTM), which takes a natural language description of the problem and produces candidate programs, none of which are correct but are likely to contain ingredients of a correct solution.    The second step is to use component-based synthesis (CBS), in which expressions and operators derived from the GPT-3 output are combined in the style of enumerative synthesis, until a solution that passes the input output examples is obtained.  

The use of PTM itself requires presenting to the system a carefully constructed “prompt” which increases the chance of the pre-trained model producing a useful output.

The CBS phase is basically a beam search approach, but it draws upon the output of PTM in three ways:  (1) to gather initial ingredients (components) which to combine, (2) obtain guidance on the operators to be used for combining components, based on their distribution in the PTM output, and (3) ranking solutions based on their closeness to PTM output.

The paper shows results in the regex domain that outperform the previous state-of-the-art (a 2020 paper).  It also shows the overall approach applies to a different domain - that of CSS selectors.   The paper finishes with a discussion on limitations, and in fact shows why the same approach does not  carry over easily to the Pandas domain.

Strengths and Weaknesses
------------------------
Why I liked this paper?

There are several items of novelty in the paper, which make it interesting.

1. AFAIK, there hasn’t been much academic paper published on program synthesis using GPT-3, and this might well be the first. (However, this is a fast moving target, and the world may be just days or weeks away from seeing one appear somewhere!)

2. It shows two interesting things in that regard:
    a. Formulating the prompt wisely
    b. And using the PTM output to guide all phases of CBM, assuming that something about the PTM output is “in the ballpark”.  The overall gadget of using enumerative synthesis with prioritization is done in many ways, but this might be the first to do it based on PBM.

I liked that the paper did point to some limitations when going to an additional domain (Sec 7, Pandas.)

Main weaknesses

1. The domain-agnostic success of the approach may be oversold (see comments further below.)
2. The act of prompting the GPT-3 model using very-related questions might be an unfair advantage, depending on the domain we are using this system for, and it may be an unreasonable way of using the system.
3. I would have liked to see some more empirical validation on how well the PTM predictions contain “good” ingredients for the eventual solution, and do not contain useless ingredients.  (This point seems to me the main takeaway of the paper.)

This is not a weakness of the paper, but given the number of DSL-based papers in synthesis, and already some successes, I would have liked to see how well this kind of approach (that uses GPT-3) can work with more general coding tasks.

Comments for author
-------------------
1. Granted that GPT-3 is very new, aren’t there other papers, even informal, that should be mentioned in the Related Work in the space of code generation based on GPT-3?  
What about https://arxiv.org/pdf/2105.09938.pdf ?  


2. Many enumerative synthesis papers employ some sort of prioritization strategy (e.g. using weights in TF-Coder paper LINK).  Here the prioritization is derived from the output of the PTM model.   This last assumption should be validated independently because this seems to be the essential nugget that can be leveraged in follow up research on this topic. (This is notwithstanding the issues already found in Sec 7.).   An ideal (but hypothetical) PBM output would contain a small number of terms and operators that are needed in the solution.  How far from ideal did we get for various problems ?


3. Given additional positive and negative examples, couldn’t the synthesizer get more specific information that it can use to guide the search (e.g. additional pruning along unpromising paths) ?


4. Sec 4 bothers me.  Why do we need to provide similar questions as a prompt?  Is this realistic in a domain-agnostic approach?  Also, if the prompt was populated by the same 3-4 canned examples, followed by the specific question, how much does the overall effectiveness drop ?  (See #7 below also.)


5. In Sec 5.1.2 I am not sure why this is an argument to support domain-agnostic approach.  This is more a problem with Regel in that it might be somewhat overfitted to the DeepRegex suite.   Also, it is not reported why Regel did not do so well on the Stack Overflow suite: was sketch generation the issue or was the subsequent phase the issue?


6. I felt that the domain-agnostic success of this paper is a bit oversold.  We have seen results on just two domains, and have seen that the idea does not work on a different domain (Sec 7.). 


7. I am puzzled why the BFS performance is pretty good in the CSS case study but not so good in the Regex case study.   I would have expected BFS to do not so poorly across the board, because it does pick its ingredients from PTM predictions (at least one time.).   I am not sure how the authors could inspect this further, but I wonder if somehow picking the right prompt is giving NLX an unfair advantage in the Regex case study.

Questions for authors’ response
---------------------------------
I would like the authors to respond to my comments #4, #5, and #7; and I would urge the authors to think about #2 and make their paper more valuable.



Review #410C
===========================================================================

Overall merit
-------------
5. Strong accept

Review confidence
-----------------
3. High

Paper summary
-------------
This work describes an approach for using “few-shot learning” to guide a synthesizer’s exploration of the program space.  The input to the synthesizer is multi-modal in that it includes both a natural language description of the target program and a set of input-output examples.  “Few-shot learning” takes advantage of a pre-trained generative natural language model (e.g., GPT3) to suggest answers for a tool-provided prompt.  (E.g., if the tool provides 10 examples of regular expression descriptions in natural language followed by the target regular expressions, and then a natural language description for the regular expression to synthesize, the language model can guess a number of plausible regular expressions.)  The technique described in this paper uses the outputs of the few-shot learning *not* as the final programs but as a set of input programs from which to mine components.  In particular, the technique (i) finds large repeated components to use to initialize synthesis, (ii) finds common operators to use to recombine components to produce larger programs, and (iii) ranks programs that satisfy the provided input-output examples based on similarity to the language model’s output programs.

Comments for author
-------------------
**Technical Details and Presentation**

Multi-modal specification is a promising direction.  The motivating examples in 1.1 provide good intuition for why a combination of modes can help users disambiguate.

Mining the GPT-generated programs for large common subcomponents is an elegant approach for integrating the few-shot learning information into the synthesis process, in keeping with the now-standard approach of using machine-learned components to guide a standard synthesizer in navigating the program space.

It’s interesting that the approach for guiding the search based on the few-shot learning actually extracts information for all of initialization, expansion, and ranking from the same query to the learned model (the single NL query -> suggested programs result).

How dependent is the system on how ‘similar’ (quotes since I provide no definition for similarity here) the training-time NL queries are to the users’ plausibly quite different NL queries?  It seems plausible that this could work well for a suite of NL prompts with similar style, pulled together by the research team (and used for the initial few-shot learning query), but fail to work nicely for users’ more diverse prompts.

Relative completeness is interesting, but doesn’t get at the core question here.  I’m not worried that the synthesis part of the process will fail to explore the space of programs--we’re worried that the machine learning part of the process will fail to provide the necessary constructs.  So unfortunately relative completeness is still unsatisfying.

Is the prompt in Figure 5 the exact query used to get the set of plausible programs?  Constructing this query could be one of the most sensitive parts of this process.  (Making the domain-specific query could also make it hard to extend the work to additional domains, despite the paper’s claims about domain-independence.)  This is ultimately explained in Sec 4, but it would help to see more detail earlier.

“If the distance is less than a threshold �� then the answers are considered too close and the question-answer pair is discarded. This is to ensure that the PTM is not biased toward a particular group of tasks and does not produce sub-optimal results.”  How did the authors realize/observe this in the first place?  Very interesting.  Why does the similarity check actually hurt for $R_{TM}$?  Why is that outcome worse than random?  Great discussion in 4.1.2, and I’d love to see more on this topic.

**Evaluation**

BFS -- a very useful, non-strawman point of comparison.  Seeing the comparison to this naive way of integrating the few-shot learning inputs was very helpful for evaluating the techniques in the paper.

I would have loved to see variants on the BFS baseline.  I.e., NLX-Reg without initialization, without expansion, without ranking.  This would help to understand whether *all* of these techniques were really required.  I’m particularly interested in whether expansion really improved performance, but I think all three would offer interesting insights.

Why was the prompt generation approach not evaluated further?  (That is, further than in 4.1.)  For instance, why was it not compared against using a single hand-crafted prompt for all tasks in a given domain?

Section 5 also increases my concern about the sensitivity to prompt generation.  If the DeepRegex test (respectively, the StackOverflow test) pulled on training data from only the DeepRegex dataset (respectively, the StackOverflow dataset), then it’s not just making one prompt/prompt template for a given domain but for *slices* of each given domain.  This makes it much harder than the introduction suggests to generalize this approach, since we seem to still need a small- to medium-sized body of input-output examples to do “training” (prompt generation), even though we’re using pre-trained models.  It’s reasonable to promote the domain independence in comparison to a tool like Regel, but the introduction overpromises a bit.

Overall, I would have loved to see more variants explored.  E.g., what other plausible ways might the tool extract guidance for rankings?  Incorporating string similarity is interesting, but what are other points in this space?  But I understand that limited space limits how much of this kind of exploration is possible in one paper.

**Discussion**

The discussion in Section 7, and especially the discussion of assumptions (C) and (D), is extremely valuable.  I appreciated that the authors included this discussion of limitations and in particular the concrete examples in Fig. 11 that give intuition for why (C) and (D) may not apply across domains.

**Summary**

This work presents an interesting technique with exciting new directions for using learned models to direct a synthesizer’s search through the program space.  I expect it will prompt interesting conversations at the conference.

==> opt.tex <==
\section{Optimized use of the PTM}
\label{sec:opt}


We have described how our generic component-based synthesis technique uses
the top candidate results of a PTM to guide the search towards the correct
program that satisfies the examples.
%
However, the effectiveness of this process depends very much on the quality
of the initial results received from the PTM, and in this section we discuss
how to best leverage the PTM we use for this purpose.
%
\arsays{These following 3 sentences should probably be in the intro.}
%
After being trained on a sufficiently varied text corpus, PTMs such as GPT-3
are able to perform a “surprising amount of tasks without the need for
explicit supervision”.
%
However, part of the versatility of these models is due to the
\emph{in-context} learning that is provided at runtime when being used for a
particular application \cite{brown2020language}.
%
This prompt (the context) helps to focuses attention on the relevant part of
the large pre-trained space that the model is searching within.
%
In the case of GPT-3, this prompt has a size limit of 2048 tokens (around
~1500 words), and an open question is how one best uses this limited space
for the application at hand.

\COM{GS: we may want to first say that we performed a formative study to
evaluate GPT-3 in the context of NL to regex. Then we can describe the
findings?}
%
Our findings demonstrate that the content of this context has a significant
impact on the responses that are returned from GPT-3, and that through
leveraging creativity and techniques from Information Retrieval, the
candidate responses from GPT-3 can be significantly improved.
%
\COM{GS: I did not understand this part. What techniques are we talking
about? It could be good to have some examples.}
%
\COM{dm: outline ur methodology here}
%
These findings suggest that by leveraging training data in a manner similar
to other Machine Learning techniques, our recall can be improved, provided
that relevant "training data" is selected for the given testing example,
training data here referring to the examples placed into the context provided
to GPT-3.

Here we propose a consistent structure for how to create a context, and four
distinct approaches for how to utilize training set examples to form that
context.

\COM{GS: Usually, for FSE, we would have to make this study more formal and
explain why we chose these values for these variables.}
All the below results are performed at a temperature of 0.7, with 20 a
candidate set of 20 results returned from GPT-3, if any result in the
candidate set is a semantic match (on all inputs) with the ground truth, the
test is marked as successful

\COM{MR: I would say that as long as we explain the reasons for choosing
these values it should be good (e.g. no need for formal analysis of all
possible temperature values, etc). What I do note is that paragraph a bit
suddenly without any explanation of what temperature means, etc. So maybe
have it later where we actually describe the experiments after defining the
context, etc}

\subsection{Context Structure}

\COM{MR: Please start with "An example of a context given to GPT is
illustrated in Figure X...." then describe all the parts of what consitutes a
context.}

Our context begins with a description of the “meta-task” we want GPT-3 to
perform (Domain).

Followed by an arbitrary number of Question – Answer training pairs (referred
to as N), in a consistent format.
%
The utility of this is twofold.
%
The format itself means GPT-3 has a high probability to produce a response in
the same format, which provides us with a structure through which to
interpret the result.
%
Secondly, the examples provided often contain components that increase the
probability of GPT-3 returning that component.
%
Examples that are relevant to the domain and the users question are therefore
critical to get the best results.
%
Finally, our context contains an “incomplete example”, that is, the test
element we wish to generate.

//Insert example context (use latex example environement)

\subsection{Baseline Context Types}
\label{subsec:ContextTypes}

\COM{GS: we may want to split section 4 in 2 main sections: method and
results. Right now, the methodology and the results are presented at the same
time.}
\COM{MR: fully agree with GS - please talk about results only at the end
after all definitions and methodology.}

Given this structure for our context, our results indicate that the relevance
of the examples to the test question contained in the context, have a
significant impact on the results.
%
Our contribution describes two novel ways of utilizing this section of the
context(Dynamic, TF-IDF), along with two more standard approaches for
comparison (Static, Random).
%
// we describe the
baseline here and 4.3 outlines the other approaches

\begin{itemize}
    \item Static Context: 
    We randomly select a set of N (where N is the maximum number of examples
    that can fit into the prompt’s maximum size of 2048 tokens, in the range
    of 5-50) examples from the training set, parse these into our context
    format, and utilize them for every question in the test set.
    %
    \item Random Context: 
    The N examples from the training set are selected randomly, however in
    this case a new random set is selected for every testing element rather
    than the same set being used throughout.
    %
    Training example sets may overlap without penalty.
    %
    The efficacy of this approach varies depending on the ratio of the number
    of examples selected vs against the total size of the training set.
\end{itemize}

\subsection{Selecting the Most Relevant Examples}

With our approach, the examples selected from the training set to be provided
in the prompt to GPT-3 are intentionally curated to be relevant to the user’s
question.

The idea here being that many of the examples in the training set will
contain components that are relevant to the test element in question, and by
selecting the most relevant examples from the training set, we provide the
best “building blocks” to GPT-3 in the hope that is it is able to assemble
these appropriately to generate an expected response.
%
We propose two techniques for the selection of these "most relevant
examples".

// Talk about a particular example here

Our approach is based on the hypothesis that certain training are more relevant
to a given test input than others.
%
For example, for the test input ``Get me all the vowels and numbers'', the
training example ``Get me all the vowels'' is more relevant than ``Match all
special characters''.
%
To determine relevance, we are guided by standard IR principles: n-gram match
and TF-IDF retrieval.
%
The two approaches detailed below are each based on one of these principles.



\label{subsec:ContextTypes}
\subsubsection{Dynamic Selection}
// just outline the procedure here, as you'll have added the example above
// describe what the n-gram is, split words by space essentially

All relevance is based off the currently selected test question.
%
The Question is split into its compositional n-grams of size 1, based on word
boundaries.

Example: “Lines containing the string ‘b’” would be decomposed into:
[``lines'',``containing'',``the'',``string'', ``’b’'']

The training set is then taken, partitioned by each example, and split into
n-grams in the same manner as above.

The average number of overlapping n-grams per example is then calculated, so
as to not bias towards longer examples with more words

The examples in the training set are then ranked in a descending manner by
the largest number of average overlapping n-grams.
%
The top N ranked values are then selected to be contained within our “dynamic
context”.
%
This process is repeated for each question in the test set.

We define dynamic relevance as follows:
\[
 \mathsf{Relevance}_\mathsf{dyn}(\mathsf{example}_\mathsf{test},
\mathsf{example}_\mathsf{train}) =
     \frac{| \mathsf{NGrams}(\mathsf{example}_\mathsf{test}) \cap \mathsf{NGrams}(\mathsf{example}_\mathsf{train}) |}{ \mathsf{Length}(\mathsf{example}_\mathsf{train}) }
\]
%
Given this relevance function, we rank the training examples
by decreasing relevance and pick the top $n$ examples to build
the context for GPT-3.

\subsubsection{TF-IDF Selection}
The TF-IDF principle assigns a score to each n-gram based on its frequency in
the corpus of training inputs.
%
We use an off-the-shelf TF-IDF vectorizer (scikit-learn ...) to produce the
scores: it takes as input the set of training example inputs and produces a
corpus of $n$-grams of different lengths along with their scores.
%
Let us denote these scores using the function $\mathsf{Score}_{tfidf}$.
%
Now, given a test input and a training input, we use the vectorizer to produce
n-grams for each and take their intersection to get the common n-grams.
%
The TF-IDF relevance of the training input to the test input is given by the sum
of the $\mathsf{Score}_{tfidf}$ values for the common n-grams, divided by the
length of the training input.
%
Add formula here.
%
However, using this relevance function as is leads to selection of very similar
training examples.

\begin{example}
   Add scenario with vowels and stop words
\end{example}

Therefor, we additionally use the Levenstein distance to avoid selecting
training examples that are too similar to each other.
%
More precisely, we start with the top ranked training example.
%
In each step, we pick the next example according the rank, and only add it to
the context if its Levenstein distance to all examples already in the context is
greater than a threshold.
%
In the experiments, we use the threshold value $x$.

\begin{example}
   Continuing from Example~\ref{ex:..}, applying the additional selection
   procedure based on Levenstein distance produces the following context.

   Compared to the context produced in Example~\ref{ex:...}, this context has
   more variety.
   %
   Hence, ..
\end{example}

\subsubsection{TF-IDF Selection}
This approach, based off of Term Frequency, Inverse Document Frequency
(TF-IDF) \cite{sparckjones1972} aims to include examples within the context
that are most relevant to the test element.
%
However in contrast to the “dynamic” approach which is naïve in nature,
focusing exclusively on overlapping N-Grams.
%
This approach builds on the learnings from previous NLP works.
    
In this approach we take the training corpus and run a TF-IDF vectorisor on
it \cite{scikit-learn}.
%
This returns us the relative TF-IDF scores of each element in the corpus.

The test element is then used to filter which elements in the corpus are
relevant, only words contained within the test element or that are synonyms
of those words are searched for in the corpus.

The relative scores of the relevant entries are then calculated, examples are
ranked descending based on the highest TF-IDF overlap scores with the test
element.
%
The top N entries are then selected to be contained with the context.

Due to a number of very similar Regular Expressions in the training set and
in order to facilitate variety in the context’s regular expressions, as the
elements are added to the context, they are checked to ensure that no Regular
Expression which has already been added to the context is within 1
Levenshtein distance [ref] of the new example to be added.
%
If so, the example is skipped and the process continues until the context has
reached capacity (N).
%
This process is repeated for every question within the test set.

\label{subsec:Context Results}

\begin{figure}
 \begin{tabular}{||c c c c||} 
 \hline
 ContextType & N & Correct Candidates &  \% Correct \\ [0.5ex] 
 \hline\hline
 Static & 35 & 33 & 28.45 \\ 
 \hline
 Random & 35 & 40 & 34.48 \\
 \hline
 Dynamic & 5 & 51 & 43.97 \\
 \hline
 Dynamic & 35 & 56 & 48.28 \\
 \hline
 Dynamic & Max(~50) & 57 & 49.14 \\ [1ex] 
 \hline
 TF-IDF & 5 & 49 & 42.24 \\
 \hline
 TF-IDF & 35 & 57 & 49.14 \\
 \hline
 TF-IDF & Max(~50) & 59 & 50.86 \\ [1ex] 
 \hline
\end{tabular}
\caption{Breakdown of recall in top 20 candidates by Context Type sent to GPT-3. Dynamic - Examples selected based on N-grams of 1, TF-IDF - Examples selected based on TF-IDF and Levenshtein distance, MAX indicates selection of the maximum number of examples capable of fitting into the prompt for each element}
\label{tab:table-name}
\end{figure}

\begin{figure}
\includegraphics[width=0.32\textwidth]{Figs/plot.pdf}
\caption{Visual showing Percentage recall in 20 candidates by Context Type sent to GPT-3}
\end{figure}


\subsection{Context Conclusions}
\label{subsec:Context Conclusions}
The above results in Fig. \ref{tab:table-name} show two key trends:
%
That the utilization of “intelligence” within the domain of context-creation
for GPT-3 increases the quality of the returned result set.
%
We can see this shown in the data from taking a strictly naive approach with
a static context, to taking a more “generalized” naive approach with the
random context.
%
Up to the Dynamic and TF-IDF contexts which leverage the content of the
user’s question with increasing smartness.

Secondly the number of contextual examples is less important that the quality
of those examples.
%
As we see diminishing returns in the impact of each added example.
%
In the dynamic context case we see that 5 dynamically selected examples
outperforms 35 selected on a random basis.
%
Adding up to an additional 15 examples on average provided only one
additionally correct candidate.


==> pandas.tex <==

%\subsection{Case study: Python Pandas}
%\label{subsec:pandas}

Pandas is a data processing library built on top of the Python programming language.
It is popular among data scientists for writing scripts that can be used to 
ingest data into a dataframe, clean it, reshape and manipulate data, and visualize it.
Pandas is a good target for generating code from NL descriptions because 
(a) it is widely used, including by non-programmers, and 
(b) it has a very large API, and it is very difficult to remember the API details, especially
for an occassional user.

Since Pandas is a large library, generating Pandas code is more challenging than generating
code in more niche (sub)languages, such as regular expressions and CSS selectors. 
Here, by generating code, we mean code that the {\em{user would have written themself}}, and not
{\em{some code that would accomplish the user's task}}. The distinction is important, since we want
the generated code to be {\em{readable}} and {\em{understandable}} by the user, which enables the
user to {\em{edit}} or {\em{adapt}} the code to their needs. Consequently, the DSL here is the
grammar for Python that includes the 100s of methods defined in the Pandas library for working
with dataframes, series, and so on.\footnote{In particular, we are not interested in synthesizing code in a hand-crafted abstract language, and then producing Pandas code via code generation.} 
\COM{GS: I am sure if the readability discussion adds much here. If we are focusing on pandas, it seems natural that the DSL will include pandas' methods.}
%
%We did some preliminary experiments on generating readable Pandas code from NL descriptions, and found that
%the combination of PTM and component-based synthesis is very valuable. The learnings from the other domains
%carry over to this domain. However, there are a few differences %in this domain.

Thus, there are two key challenges in this domain. First, the DSL is very large since it includes all of the available methods in the Pandas API.
Second, there is no fixed input domain and output domain that works for all terms -- 
the input and output domains vary across all possible programs, and hence, there is no
universal notion of examples that a user can provide.
%Consequently, the proposed approach is not directly applicable, but it can be adapted to provide
%{\em{one step}} in the overall pipeline for generating Pandas code from user's intent expressed in NL.  
\input{Figs/Pandas}

Given the above challenges, we can not use the {\textsc{nlx}} algorithm directly here, but we can verify if the hypothesis underlying the approach holds, namely, whether
the candidates generated by the PTM contain the components needed to generate the ground truth.
%We discuss some concrete case studies, shown in Figure~\ref{fig:pandasexamples}, to illustrate the value of component-based synthesis can bring in this domain.
%
We collected NL descriptions 
\COM{MR: while this is good that we have few hundred, it feels very weird that we collected so many for this case study where we had not implementation and so little for css where we did have an implementation. Maybe we dont mention this (because the hundreds were for reasons not related to this paper) and say we looked at a few cases.}
along with ground-truth expressions
from stackoverflow posts about Pandas. We then used a PTM to generate 25 candidate programs
for the NL descriptions. We then analyzed if the candidates have the components used in the
ground-truth program.  We used dynamic prompt generation. There were around 40\%\COM{GS: the use of a few and around may be too informal} benchmarks where the
ground-truth program was present in the 25 candidates. Figure~\ref{fig:pandasexamples} shows three instances When the ground truth was not present in the candidates returned by PTM. There were three classes of instances.
In the first class, the candidates contained all components used in the ground truth.
For example, consider the ground-truth program 
$\text{df.groupby(['HP', 'Type 1']).agg(['mean', 'count'])}$ 
that corresponds to the NL description "group by HP and Type 1 and calculate mean and count for each group"\COM{GS: do we have the link for the stackoverflow post for this example?}.  Among the generated candidates, we find the maximal components
$\text{df.groupby}$,
$\text{['HP', 'Type 1']}$,
$\text{agg}$, 
$\text{np.mean}$, and
$\text{'count'}$, which can be combined to give the program
$\text{df.groupby(['HP', 'Type 1']).agg([np.mean, 'count'])}$,
which is equivalent to the ground-truth program. 

The other two examples in Figure~\ref{fig:pandasexamples} show cases where the
candidates do not contain all the components needed to recreate the ground truth, but 
they contain many of the components. In the first row, only one component, namely
$\text{set\_index}$ is missing. This is quite common, and our component-based synthesis approach can find the desired program for such cases.  In the last row, a few components are missing, namely
$\text{to\_series}$, $\text{df.dtypes}$, and $\text{groups}$.  When more than one component
is missing, it is difficult for component-based synthesis to generate the intended program,
and we need other methods to repair the PTM output, such as, the use of types to suggest repairs, which we leave for future work.
\COM{MR: rather than simply say other methods are needed, may be good to discuss possible solutions as future explorations to build upon the work here}
\COM{GS: also, it is strange that we are saying that it is hard to use synthesis for these 2 examples when we actually did not use synthesis in any of the examples. I think we have to discuss a little bit more how we could use synthesis then.}

The combination of PTM and component-based synthesis, however, are a vital part\COM{GS: vital part sounds very strong. In special when we do not show any use of examples in this domain.} of the 
pipeline for generating Pandas code from NL descriptions.



